Scal3R: Learning Efficient Multi-Relative Pose Query for Scalable Online 3D Reconstruction

Online 3D reconstruction models perform poorly on long videos. This happens because regressing poses relative to a fixed first-frame anchor forces extrapolation far beyond the training distribution. Small drifts accumulate and amplify into significant geometric collapse. However, we observe that per-frame depth remains stable throughout this failure. The backbone's local geometry remains intact; only the global pose head breaks down. Motivated by this decoupling, we introduce Scal3R. This approach reformulates online reconstruction as multi-reference relative pose querying. We use lightweight learnable tokens, which make up about ~1% of the parameters, and inject them into a completely frozen backbone via asymmetric attention. This setup queries poses relative to multiple past keyframes. An online pose-graph optimization system with loop closure suppresses long-range drift. Scal3R reaches convergence in 8 hours on a single GPU. It reduces the average ATE by over 60% on KITTI compared to the online baseline. It also achieves state-of-the-art performance across Virtual KITTI, Sintel, TUM-Dynamic, ScanNet, and 7-Scenes. Project page: https://linjohnss.github.io/scal3r/

==> tables/sintel_tum_scannnet.tex <==
\begin{table}[t]
  \caption{\textbf{Quantitative evaluation on Sintel, TUM-RGBD, and ScanNet.} We report the Absolute Trajectory Error (ATE $\downarrow$) for various methods. Scal3R (Ours) consistently outperforms existing streaming architectures, achieving state-of-the-art precision in dense indoor environments like ScanNet.}
  \label{tab:sintel_tum_scannet_results}
  \centering
  \resizebox{\columnwidth}{!}{
  \begin{tabular}{l ccc}
    \toprule
    \multirow{2}{*}{\textbf{Methods}} & \textbf{Sintel} & \textbf{TUM} & \textbf{ScanNet} \\
    \cmidrule(lr){2-2} \cmidrule(lr){3-3} \cmidrule(lr){4-4}
    & \textbf{ATE} $\downarrow$ & \textbf{ATE} $\downarrow$ & \textbf{ATE} $\downarrow$ \\
    \midrule
    MASt3R-SLAM \cite{murai2025mast3r} & 0.233 & 0.103 & 0.081 \\
    MUSt3R \cite{cabon2025must3r} & 0.242 & 0.048 & 0.046 \\
    CUT3R \cite{wang2025continuous} & 0.210 & 0.049 & 0.095 \\
    Point3R \cite{wu2025point3r} & 0.375 & 0.067 & 0.120 \\
    STream3R \cite{lan2025stream3r} & 0.214 & 0.026 & 0.052 \\
    WinT3R & 0.225 & 0.074 & 0.062 \\
    StreamVGGT \cite{streamVGGT} & 0.394 & 0.057 & 0.120 \\
    TTT3R \cite{chen2025ttt3r} & 0.210 & 0.028 & 0.064 \\
    \midrule
    \textbf{Ours (CUT3R)} & \textbf{0.168} & 0.033 & 0.092 \\
    \textbf{Ours (STream3R)} & 0.171 & \textbf{0.018} & \textbf{0.018} \\
    \bottomrule
  \end{tabular}
  }
\end{table}

==> tables/vkitti.tex <==
\begin{table}[t]
  \caption{\textbf{Quantitative comparison on the Virtual KITTI (vKITTI) dataset in terms of ATE $\downarrow$.} The upper block lists offline baselines, the middle block reports online methods, and the lower block presents our Scal3R variants. Our approach demonstrates superior robustness on long-range sequences (e.g., Scene 20), achieving state-of-the-art accuracy among all streaming-based architectures. \textbf{-} denotes out-of-memory (OOM) or tracking failure.}
  \label{tab:vkitti_final_refined}
  \centering
  \resizebox{\textwidth}{!}{
  \begin{tabular}{l ccccc | c}
    \toprule
    \multirow{2}{*}{\textbf{Methods}} & \multicolumn{5}{c}{\textbf{vKITTI (ATE $\downarrow$)}} & \multirow{2}{*}{\textbf{Avg.}} \\
    \cmidrule(lr){2-6}
    & \begin{tabular}[c]{@{}c@{}}Scene01\\ \scriptsize{447x, 1.3km}\end{tabular} & \begin{tabular}[c]{@{}c@{}}Scene02\\ \scriptsize{233x, 0.6km}\end{tabular} & \begin{tabular}[c]{@{}c@{}}Scene06\\ \scriptsize{270x, 0.6km}\end{tabular} & \begin{tabular}[c]{@{}c@{}}Scene18\\ \scriptsize{339x, 1.1km}\end{tabular} & \begin{tabular}[c]{@{}c@{}}Scene20\\ \scriptsize{837x, 2.5km}\end{tabular} & \\
    \midrule
    VGGT \cite{wang2025vggt} & - & 0.219 & - & - & - & 0.219 \\
    Fast3R \cite{yang2025fast3r} & 72.708 & 23.716 & 6.049 & 58.929 & 159.402 & 64.161 \\
    DA3 \cite{lin2025depth} & 25.216 & 0.216 & 0.167 & 12.530 & 182.888 & 44.203 \\
    $\pi^3$ \cite{wang2025pi} & 4.629 & 0.330 & 0.176 & 3.039 & - & 2.044 \\
    \midrule
    MASt3R-SLAM \cite{murai2025mast3r} & 75.156 & - & 7.056 & - & - & 41.106 \\
    MUSt3R \cite{cabon2025must3r} & 77.226 & 7.389 & 0.280 & 48.528 & 170.906 & 60.866 \\
    CUT3R \cite{wang2025continuous} & 59.764 & 29.729 & 0.649 & 44.888 & 146.920 & 56.390 \\
    Point3R \cite{wu2025point3r} & 75.695 & 30.440 & 4.811 & 62.846 & 138.240 & 62.406 \\
    STream3R \cite{lan2025stream3r} & 66.831 & 25.466 & 1.524 & 68.181 & 223.070 & 77.014 \\
    WinT3R & 59.019 & 28.606 & 1.102 & 42.893 & 203.159 & 66.956 \\
    StreamVGGT \cite{streamVGGT} & 55.093 & 32.906 & 0.569 & 57.181 & - & 36.437 \\
    TTT3R \cite{chen2025ttt3r} & 29.053 & 12.149 & 0.535 & 6.749 & 77.900 & 25.277 \\
    \midrule
    \textbf{Ours (CUT3R)} & \textbf{4.496} & \textbf{0.717} & \textbf{0.664} & \textbf{5.559} & \textbf{16.722} & \textbf{5.632} \\
    \textbf{Ours (STream3R)} & \textbf{5.393} & \textbf{3.259} & \textbf{3.210} & \textbf{6.400} & \textbf{21.322} & \textbf{7.917} \\
    \bottomrule
  \end{tabular}
  }
\end{table}
